Construction and Iteration-Complexity of Primal Sequences in Alternating Minimization Algorithms

We introduce a new weighted averaging scheme using "Fenchel-type" operators to recover primal solutions in the alternating minimization-type algorithm (AMA) for prototype constrained convex optimization. Our approach combines the classical AMA idea in \cite{Tseng1991} and Nesterov's prox-function smoothing technique without requiring the strong convexity of the objective function. We develop a new non-accelerated primal-dual AMA method and estimate its primal convergence rate both on the objective residual and on the feasibility gap. Then, we incorporate Nesterov's accelerated step into this algorithm and obtain a new accelerated primal-dual AMA variant endowed with a rigorous convergence rate guarantee. We show that the worst-case iteration-complexity in this algorithm is optimal (in the sense of first-oder black-box models), without imposing the full strong convexity assumption on the objective.

==> TranDinh_OptLetter2015_impl.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 8. Applications and numerical experimence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3ex}
\section{Implementation remarks and numerical verifications}\label{sec:impl_aspects}
\vspace{-2ex}
We first discuss some implementation aspects of Algorithms \ref{alg:pd_ama} and \ref{alg:pd_ac_ama}. Then, we provide two numerical examples to verify our theoretical results.

\vspace{-3ex}
\subsection{Comments on the implementation}
\vspace{-2ex}
First, when $g$ and $h$ are not strongly convex, Algorithms \ref{alg:pd_ama} and \ref{alg:pd_ac_ama} require smoothing prox-function $p$ for $\Uc$.
Depending on the structure of $\Uc$, we can choose an appropriate prox-function $p$ such that the computation of $\hat{u}^{k+1}$ in \eqref{eq:ama_scheme} is efficient.
For instance, if  $g_{\Uc} = g + \delta_{\Uc}$ has a tractable proximity operator, we can choose $p(\ub) := (1/2)\norm{\ub-\ub_c}^2_2$ for a given $\ub_c\in\Uc$. 
If $\Uc$ is a standard simplex, then a negative entropy prox-function $p$ is the optimal one.

Second, the choice of smoothness parameter $\gamma$ in Algorithms \ref{alg:pd_ama} and \ref{alg:pd_ac_ama} is also crucial to trade of the performance of these algorithms.
Theoretically, this parameter is fixed a priori. However, in practice, we can adaptively decrease this parameter to avoid a slow convergence.
We can either use fixed the dual step-size using the dual Lipschitz constant $\gamma^{-1}L_{d^1}$ or adaptive step-size via a line-search procedure.
We can also inject an adaptive restart strategy \cite{Odonoghue2012} into Algorithm~\ref{alg:pd_ac_ama} to accelerate its practical performance.

Finally, when $\Bb$ is not orthogonal, the computation of $\hat{\vb}^{k+1}$ in \eqref{eq:ama_scheme} requires to solve a general convex subproblem.
As done in preconditioned techniques \cite{Chambolle2011}, we can linearize the quadratic term in order to exploit the tractable proximity of $h_{\Vc}$.

\vspace{-3ex}
\subsection{Numerical verifications}
\vspace{-2ex}
We verify the bounds given by Algorithms~\ref{alg:pd_ama} and \ref{alg:pd_ac_ama} in Theorem \ref{th:primal_recover1} and \ref{th:primal_convergence2}, and Corollary \ref{co:primal_convergence1b} using the following simple projection problem on a polytope:
\begin{equation}\label{eq:qp_exam}
g^{\star} := \min_{\ub\in\R^{p_1}}\left\{ g(\ub) := (1/2)\norm{\mathbf{D}\ub -\mathbf{q}}^2_2 : \mathbf{a} \leq \Ab\ub \leq \mathbf{b}, \norm{\ub}_{\infty} \leq r \right\}.
\end{equation}
where $\mathbf{D} \in\R^{p_1\times p_1}$ is a diagonal positive (semi)definite matrix, $\mathbf{q}\in\R^{p_1}$,  $\Ab\in\R^{n\times p_1}$, $\ab, \bb\in\R^n$ such that $\ab < \bb$, and $r > 0$.
By introducing a slack variable $\vb = \Ab\ub$, and the indicator function $h(\vb) := \delta_{\set{\ab\leq\vb\leq \bb}}(\vb)$, we can reformulate \eqref{eq:qp_exam} into \eqref{eq:constr_cvx} with $\Uc := \set{\ub\in\R^{p_1} : \norm{\ub}_{\infty} \leq r}$ and $\Vc := \set{\vb\in\R^n: \ab \leq \vb\leq \bb}$.

Matrix $\mathbf{A}$ is generated randomly using i.i.d. samples from the standard Gaussian distribution $\mathcal{N}(0, 1)$. Vectors $\mathbf{a}$ and $\mathbf{b}$ are generated as $\mathbf{a} := \Ab\xb^{\natural} - \mathbf{R}(0,1)$ and $\mathbf{b} := \Ab\xb^{\natural} + \mathbf{R}(0,1)$, where $\xb^{\natural}$ is a given i.i.d. Gaussian random vector, $\mathcal{R}(0,1)$ is a vector of uniform random numbers. The diagonal matrix $\mathbf{D}$ and vector $\mathbf{q}$ are also generated randomly such that $\mathbf{D}\succeq 0$.
In the strongly convex case, i.e., $\mathbf{D}\succ 0$, we choose $r = \infty$, while in the non-strongly convex case, we use $r = \norm{\xb^{\natural}}_{\infty}$.

In order to compute the theoretical bounds in Theorems \ref{th:primal_recover1} and \ref{th:primal_convergence2}, and Corollary \ref{co:primal_convergence1b}, we use CVX \cite{Grant2006} to solve \eqref{eq:qp_exam} up to the best accuracy. We use the CVX dual solution and objective value to compute the right-hand side bounds in our theoretical results. 

\vspace{-3ex}
\subsubsection{Theoretical bounds vs empirical performance in the non-strongly convex case}
\vspace{-2ex}
When $\mathbf{D}$ is positive semidefinite, \eqref{eq:qp_exam} is not strongly convex, we apply Algorithms \ref{alg:pd_ama} and \ref{alg:pd_ac_ama} to this case, where we fix $\eta_k := \frac{\gamma}{\norm{\Ab}^2}$ for $k\geq 0$, and $\gamma > 0$ is our smoothness parameter.

\vspace{-3ex}
\subsubsection{Theoretical bounds vs empirical performance in the strongly convex case}
\vspace{-2ex}
We consider 
